Who Uses Personas in Requirements Engineering: The Practitioners' Perspective

Personas are commonly used in software projects to gain a better understanding of end-users' needs. However, there is a limited understanding of their usage and effectiveness in practice. This paper presents the results of a two-step investigation, comprising interviews with 26 software developers, UI/UX designers, business analysts and product managers and a survey of 203 practitioners, aimed at shedding light on the current practices, methods and challenges of using personas in software development. Our findings reveal variations in the frequency and effectiveness of personas across different software projects and IT companies, the challenges practitioners face when using personas and the reasons for not using them at all. Furthermore, we investigate the coverage of human aspects in personas, often assumed to be a key feature of persona descriptions. Contrary to the general perception, our study shows that human aspects are often ignored for various reasons in personas or requirements engineering in general. Our study provides actionable insights for practitioners to overcome challenges in using personas during requirements engineering stages, and we identify areas for future research.

==> Section/Todocomments.tex <==
review 1:

1. improve related works,

2. The user is criticizing the authors' sampling strategy in their study, which aims to investigate the frequency of use and current practices. The user suggests that the sampling method used (a convenience sample) may not be suitable for the descriptive nature of the research questions (RQ 1 and RQ 2), as these questions require a sample that accurately represents the population to infer the distribution of a particular behavior or practice. The user implies that the sampling method might be more appropriate for an exploratory survey, like that of RQ 3, rather than for descriptive research. The user also questions the specific population the authors intend to describe with their survey. (update RQ1 and 2)


3. add survey results in using personas %


4. update interview guide %


5. Were the questions about using personas by project type in the survey asked for all respondents? If so, this involves assuming that they know about persona use in any project, which is unlikely. (in limitations)


6. Also, how many survey respondents reported using personas themselves (Question 7 from the survey)? It is unclear why the authors omit such information when it could help answering RQ 1. with id 4%------


7. Regarding the survey questions to answer RQ 2, there was a focus on the high-level methods (ML and data analytics, data visualization, or qualitative analysis) and the human factors. However, what about *practices*, which are more fine-grained ways of working? There are no questions about that. Therefore, the only data source is the interviews, which also provided limited information.


8. In Section 4.3, what did the authors mean with “Overall, most human aspects have agreement rates above 50%, and only physical issues have agreement rates below 50%.”? Does it mean that people use personas or not?  %%%-----


9. How were the challenges in the interviews and survey related? Given the previous information that the interviews informed the survey design, the reader can only imagine the relationship. It would be interesting to know it exactly.---------------%


10. What do the authors mean with VR-driven personas (Section 5)? ------%


11. The discussion is a list of recommendations and takeaways. They are not always clearly grounded on data (such as: “Regularly schedule collaborative sessions between software engineers/developers and the requirements analysts and product owners to discuss user needs and co-create personas”). Also, this is not a real discussion about the results, their meaning, or how they relate to previous research.


12. When discussing threats to validity (Section 6), the authors state that they invited experts in survey design and industry professionals to evaluate the survey. The authors need to report how many people participated in this. Moreover, the introduction on the initial page of the survey should be a part of the interview script.--------------------------% update guideline


13. Finally, the fact that some participants did not use personas themselves raises concerns, which should be discussed as part of the threats to validity.-------%%%



14. It is surprising to note that the paper states that personas are rarely used in VR and game design whereas these applications almost always provide a persona-based interface. The paper misses mention of mobile apps as a key category of applications that need to take personas into consideration to provide a personalized experience to users especially with the current trend of hyper-personalization---------%%


15. Although the Research Questions specifically aim to cover these three aspects and describe the interview set up and process at length, they do not analyze the current practices in persona creation and usage in any detail. No methods are presented, analyzed or compared. The data collected presents a broad classification of organizations, projects, and job profiles that use personas which gives a superficial view instead of an in-depth analysis of current practices.------%


16. The study would be more effective if it covered details of existing techniques for capturing personas, attributes captured, their utility and missing information that could serve as a guide to teams desiring to use personas.

17. Challenges in use of personas too are discussed in qualitative terms. It would help to show examples and provide some quantification. ----------%


18. Improve abstact. 


Matthews, T., Judge, T., & Whittaker, S. (May 2012). How do UX designers and professionals actually perceive and use personas? In Proceedings of the SIGCHI conference on Human factors in computing systems (pp. 1219-1228).

Salminen, J., Nielsen, L., Bahloul, M., Jørgensen, RG, Santos, JM, Jung, SG, & Jansen, BJ (2022). Persona readiness: A survey instrument to measure organizational readiness for persona deployment. Information Technology and Management, 1-26.

